A transient equivalence between Aldous-Broder and Wilson's algorithms and a two-stage framework for generating uniform spanning trees

The $Aldous\text{-}Broder$ and $Wilson$ are two well-known algorithms to generate uniform spanning trees (USTs) based on random walks. This work studies their relationship while they construct random trees with the goal of reducing the total time required to build the spanning tree. Using the notion of $branches$ $-$ paths generated by the two algorithms on particular stopping times, we show that the trees built by the two algorithms when running on a complete graph are statistically equivalent on these stopping times. This leads to a hybrid algorithm that can generate uniform spanning trees of complete graphs faster than either of the two algorithms. An efficient two-stage framework is also proposed to explore this hybrid approach beyond complete graphs, showing its feasibility in various examples, including transitive graphs where it requires 25% less time than $Wilson$ to generate a UST.

==> main.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % A template for Wiley article submissions developed by 
% % Overleaf for the Overleaf-Wiley pilot which ran 
% % during 2017 and 2018.
% % 
% % This template is no longer supported, but is provided
% % for historical reference. Last updated January 2019.
% %
% % Please note that whilst this template provides a 
% % preview of the typeset manuscript for submission, it 
% % will not necessarily be the final publication layout.
% %
% % Document class options:
% % =======================
% % blind: Anonymise all author, affiliation, correspondence
% %        and funding information.
% %
% % lineno: Adds line numbers.
% %
% % serif: Sets the body font to be serif. 
% %
% % twocolumn: Sets the body text in two-column layout. 
% % 
% % num-refs: Uses numerical citation and references style 
% %           (Vancouver-authoryear).
% %
% % alpha-refs: Uses author-year citation and references style
% %             (rss).
% %
% % Using other bibliography styles:
% % =======================
% %
% % To specify a different bibiography style
% %
% % 1) Do not use either num-refs or alpha-refs in documentclass.
% % 2) Load natbib package with the options set as needed.
% % 3) Use the \bibliographystyle command to specify the style
% % 
% % Included NJD styles are: 
% %   WileyNJD-ACS
% %   WileyNJD-AMA
% %   WileyNJD-AMS
% %   WileyNJD-APA
% %   WileyNJD-Harvard
% %   WileyNJD-VANCOUVER
% %
% % or you may upload an alternative .bst file 
% % (if requested by the journal).
% %
% % Examples:
% % =======================
% %% Example: Using numerical, sort-by-authors citations.
% % \documentclass[num-refs]{wiley-article}

% %% Example: Using author-year citations and anonymising submission
% % \documentclass[blind,alpha-refs]{wiley-article}

% %% Example: Using unsrtnat for numerical, in-sequence citations
% % \documentclass{wiley-article}
% % \usepackage[numbers]{natbib}
% % \bibliographystyle{unsrtnat}

% \documentclass[serif,dvipsnames]{wiley-article}
% \usepackage[numbers]{natbib}
% \bibliographystyle{bibstyles/WileyNJD-AMS}
% \makeatletter
% \renewcommand{\@biblabel}[1]{#1.}

% % \documentclass[serif,twocolumn]{wiley-article}
% % \usepackage[super]{natbib}
% % \bibliographystyle{WileyNJD-AMA}
% % \makeatletter
% % \renewcommand{\@biblabel}[1]{#1.}
% % \makeatother

% \pgfdeclareradialshading[tikz@ball]{my ball}{\pgfqpoint{5bp}{10bp}}{%
%  color(0bp)=(tikz@ball!10!white);
%  color(8bp)=(tikz@ball!65!white);
%  color(12bp)=(tikz@ball);
%  color(25bp)=(tikz@ball!70!black);
%  color(50bp)=(black)}

% \pgfdeclareradialshading[tikz@ball]{new ball}{\pgfqpoint{12bp}{12bp}}{%
%  color(0cm)=(tikz@ball!40!white);
%  color(0.5cm)=(tikz@ball!80!white);
%  color(0.75cm)=(tikz@ball);
%  color(0.9cm)=(tikz@ball!80!black);
%  color(1cm)=(tikz@ball!60!black)} 

%  % to make possible use "myball color=..." 
% \tikzoption{my ball color}{\pgfutil@colorlet{tikz@ball}{#1}\def\tikz@shading{my ball}\tikz@addmode{\tikz@mode@shadetrue}}

% \tikzoption{new ball color}{\pgfutil@colorlet{tikz@ball}{#1}\def\tikz@shading{new ball}\tikz@addmode{\tikz@mode@shadetrue}}

% \tikzoption{ball shadow color}{\pgfutil@colorlet{tikz@ball}{#1}\def\tikz@shading{ball shadow}\tikz@addmode{\tikz@mode@shadetrue}}

% \newcommand{\ball}[4][white]{%
%     \begin{scope}[shift = {(#3,#4)}]
%       % test to decide which shading use: special one for white balls
%       % not 100% efficient: maybe it's better to use directly a custom
%       % white ball shading, but this way one could always use 
%       % "my ball color=green" say
%       \ifnum\pdf@strcmp{#2}{white}=\z@%  
%         \shade[my ball color=#2] (0.15,0.25) circle (0.4);
%       \else
%         \shade[new ball color=#2] (0.15,0.25) circle (0.4);
%       \fi
%     \end{scope}
%     \node[color=black] at (.15+#3,.25+#4) {\LARGE$\mathbf{#1}$};
%     % \node[color=black] at (.15+#3,.25+#4) {\LARGE #1};
% }

% % Add additional packages here if required
% \usepackage{siunitx}
% \usepackage{amsmath}
% \numberwithin{equation}{section}
% \usepackage{amsfonts,amssymb}
% \usepackage{hyperref}
% \usepackage{bm}
% \usepackage{tikz,tkz-euclide,pdftexcmds}
% \usetikzlibrary{arrows,shapes.geometric}
% \usetikzlibrary{positioning}
% \usetikzlibrary{automata}
% \usetikzlibrary{arrows,shapes,calc}
% \usepackage{float}
% \usepackage[ruled,vlined]{algorithm2e}
% \usepackage{verbatim}
% \usepackage{thmtools, thm-restate}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{xcolor}

% %%%%% Commands %%%%%%
% \newcommand{\com}[1]{\textcolor{red}{\texttt{giulio:} #1}}
% \newcommand{\igor}[1]{\textcolor{blue}{\texttt{igor:} #1}}
% \newcommand{\dan}[1]{\textcolor{red}{\texttt{daniel:} #1}}
% \newcommand{\V}{{V}} % vertex set
% \newcommand{\E}{{E}} % edge set 
% \newcommand{\G}{G} % graph set
% \newcommand{\T}{\mathcal{T}} % tree set
% \newcommand{\tree}{T} % tree random variable 
% \newcommand{\spatree}{\tau} % spanning tree element 
% \newcommand{\subtree}{\zeta} % subtree element 

% \newcommand{\Ssub}{S} % subtree set element 


% \newcommand{\PP}{\mathbb{P}} % Probability 

% \newcommand{\twostage}{\rm ts} % Two-stage procedure 

% \newtheorem{proposition}[theorem]{Proposition}

% \newtheorem{conjecture}[theorem]{Conjecture}
% % Update article type if known
% \papertype{Original Article}
% % Include section in journal if known, otherwise delete
% \paperfield{Journal Section}

% \title{
% A transient equivalence between Aldous-Broder and Wilson's algorithms and a two-stage framework for generating uniform spanning trees
% }

% % List abbreviations here, if any. Please note that it is preferred that abbreviations be defined at the first instance they appear in the text, rather than creating an abbreviations list.
% % \abbrevs{ABC, a black cat; DEF, doesn't ever fret; GHI, goes home immediately.}

% % Include full author names and degrees, when required by the journal.
% % Use the \authfn to add symbols for additional footnotes and present addresses, if any. Usually start with 1 for notes about author contributions; then continuing with 2 etc if any author has a different present address.
% \author[1]{Igor Nunes}
% \author[2]{Giulio Iacobelli}
% \author[1]{Daniel Ratton Figueiredo}

% % Include full affiliation details for all authors
% \affil[1]{Systems Engineering and Computer Science Program (PESC), Federal University of Rio de Janeiro (UFRJ), Rio de Janeiro, 21941-914, Brazil}
% \affil[2]{Mathematical Institute (IM)

% Federal University of Rio de Janeiro (UFRJ)

% Rio de Janeiro, 21941-909, Brazil}

% \corraddress{Daniel Ratton Figueiredo, Systems Engineering and Computer Science Program (PESC), Federal University of Rio de Janeiro (UFRJ), Rio de Janeiro, 21941-914, Brazil}
% \corremail{daniel@cos.ufrj.br}

% %\presentadd[\authfn{2}]{Department, Institution, City, State or Province, Postal Code, Country}

% \fundinginfo{This work was supported in part by research grants from CNPq (Brazil) and FAPERJ (Brazil).}

% % Include the name of the author that should appear in the running header
% \runningauthor{Nunes et al.}

% \begin{document}

% \begin{frontmatter}
% \maketitle
% \begin{abstract}
% \include{abstract}
% \end{abstract}
% \end{frontmatter}

% \include{introduction}
% \include{aldous}
% \include{wilson}
% \include{equivalence}
% \include{framework}
% % \include{lineraly_biased}

% % \section{First Level Heading}
% % Please lay out your article using the section headings and example objects below, and remember to delete all help text prior to submitting your article to the journal.

% % \begin{figure}[bt]
% % \centering
% % \includegraphics[width=6cm]{example-image-rectangle}
% % \caption{Although we encourage authors to send us the highest-quality figures possible, for peer-review purposes we can accept a wide variety of formats, sizes, and resolutions. Legends should be concise but comprehensive -- the figure and its legend must be understandable without reference to the text. Include definitions of any symbols used and define/explain all abbreviations and units of measurement.}
% % \end{figure}

% % \subsection{Second Level Heading}
% % If data, scripts or other artefacts used to generate the analyses presented in the article are available via a publicly available data repository, please include a reference to the location of the material within the article.

% % % Equations should be inserted using standard LaTeX equation and eqnarray environments, not as graphics, and should be set in the main text
% % This is an equation, numbered
% % \begin{equation}
% % \int_0^{+\infty}e^{-x^2}dx=\frac{\sqrt{\pi}}{2}
% % \end{equation}
% % And one that is not numbered
% % \begin{equation*}
% % e^{i\pi}=-1
% % \end{equation*}

% % \subsection{Document class options}

% % The \texttt{wiley-article} document class offers the following options:

% % \begin{description}
% % \item[\texttt{blind}] Anonymise all author, affiliation, correspondence
% %       and funding information.

% % \item[\texttt{lineno}] Adds line numbers.

% % \item[\texttt{serif}] Sets the body font to be serif.

% % \item[\texttt{twocolumn}] Sets the body text in two-column layout.

% % \item[\texttt{num-refs}] Uses the numerical Vancouver bibliography style; see section \ref{sec:bibstyles}.

% % \item[\texttt{alpha-refs}] Uses the author-year RSS bibliography style; see section \ref{sec:bibstyles}.
% % \end{description}

% % \subsection{Adding Citations and a References List}
% % \label{sec:bibstyles}

% % Please use a \verb|.bib| file to store your references. When using Overleaf to prepare your manuscript, you can upload a \verb|.bib| file or import your Mendeley or Zotero library directly as a \verb|.bib| file via the Add Files menu. You can then cite entries from it, like this: \cite{urmson2008autonomous,lees2010theoretical} and \cite{geiger2012we}. Just remember to specify a bibliography style, as well as the filename of the \verb|.bib|.

% % You can find a video tutorial here to learn more about BibTeX: \url{https://www.overleaf.com/help/97-how-to-include-a-bibliography-using-bibtex}.

% % This template provides two \verb|\documentclass| options for the citation and reference list style: 
% % \begin{description}
% % \item[Numerical style] Use \verb|\documentclass[...,num-refs]{wiley-article}| (Vancouver style)
% % \item[Author-year style] Use \verb|\documentclass[...,alpha-refs]{wiley-article}| (RSS style)
% % \end{description}

% % If you are submitting to a journal that uses neither of the above, then instead of specifying one of these options in the document class you should use  \verb|\bibliographystyle| to specify the appropriate \verb|WileyNJD-...| style, and load the \verb|natbib| with the appropriate options as needed. If the journal provides you with an alternative .bst file to use, please upload this first, and then specify it with the \verb|\bibliographystyle| as above.

% % \subsection{Usage Examples of \texttt{wiley-article} Options}

% % \begin{enumerate}
% % \item Using numerical, sort-by-authors citations:
% % \begin{verbatim}
% % \documentclass[num-refs]{wiley-article}
% % \end{verbatim}

% % \item Anonymised submission using author-year citations:
% % \begin{verbatim}
% % \documentclass[blind,alpha-refs]{wiley-article}
% % \end{verbatim}

% % \item Using \texttt{unsrtnat} for numerical, in-sequence citations:
% % \begin{verbatim}
% % \documentclass{wiley-article}
% % \usepackage[numbers]{natbib}
% % \bibliographystyle{unsrtnat}
% % \end{verbatim}

% % \item Using the \texttt{WileyNJD-AMA} reference style and superscript citations, two-column and serif fonts, for submission to AIChE:

% % \begin{verbatim}
% % \documentclass[serif,twocolumn]{wiley-article}
% % \usepackage[super]{natbib}
% % \bibliographystyle{WileyNJD-AMA}
% % \makeatletter
% % \renewcommand{\@biblabel}[1]{#1.}
% % \makeatother
% % \end{verbatim}

% % \end{enumerate}

% % \subsubsection{Third Level Heading}
% % Supporting information will be included with the published article. For submission any supporting information should be supplied as separate files but referred to in the text.

% % Appendices will be published after the references. For submission they should be supplied as separate files but referred to in the text.

% % \paragraph{Fourth Level Heading}
% % % Here are examples of quotes and epigraphs.
% % \begin{quote}
% % The significant problems we have cannot be solved at the same level of thinking with which we created them.\endnote{Albert Einstein said this.}
% % \end{quote}

% % \begin{epigraph}{Albert Einstein}
% % Anyone who has never made a mistake has never tried anything new.
% % \end{epigraph}

% % \subparagraph{Fifth level heading}
% % Measurements should be given in SI or SI-derived units.
% % Chemical substances should be referred to by the generic name only. Trade names should not be used. Drugs should be referred to by their generic names. If proprietary drugs have been used in the study, refer to these by their generic name, mentioning the proprietary name, and the name and location of the manufacturer, in parentheses.

% % \begin{table}[bt]
% % \caption{This is a table. Tables should be self-contained and complement, but not duplicate, information contained in the text. They should be not be provided as images. Legends should be concise but comprehensive – the table, legend and footnotes must be understandable without reference to the text. All abbreviations must be defined in footnotes.}
% % \begin{threeparttable}
% % \begin{tabular}{lccrr}
% % \headrow
% % \thead{Variables} & \thead{JKL ($\boldsymbol{n=30}$)} & \thead{Control ($\boldsymbol{n=40}$)} & \thead{MN} & \thead{$\boldsymbol t$ (68)}\\
% % Age at testing & 38 & 58 & 504.48 & 58 ms\\
% % Age at testing & 38 & 58 & 504.48 & 58 ms\\
% % Age at testing & 38 & 58 & 504.48 & 58 ms\\
% % Age at testing & 38 & 58 & 504.48 & 58 ms\\
% % \hiderowcolors
% % stop alternating row colors from here onwards\\
% % Age at testing & 38 & 58 & 504.48 & 58 ms\\
% % Age at testing & 38 & 58 & 504.48 & 58 ms\\
% % \hline  % Please only put a hline at the end of the table
% % \end{tabular}

% % \begin{tablenotes}
% % \item JKL, just keep laughing; MN, merry noise.
% % \end{tablenotes}
% % \end{threeparttable}
% % \end{table}

% % \printendnotes

% % Submissions are not required to reflect the precise reference formatting of the journal (use of italics, bold etc.), however it is important that all key elements of each reference are included.
% %\bibliographystyle{plain}
% \bibliography{sample}

% % \begin{biography}[example-image-1x1]{A.~One}
% % Please check with the journal's author guidelines whether author biographies are required. They are usually only included for review-type articles, and typically require photos and brief biographies (up to 75 words) for each author.
% % \bigskip
% % \bigskip
% % \end{biography}

% % \graphicalabstract{example-image-1x1}{Please check the journal's author guildines for whether a graphical abstract, key points, new findings, or other items are required for display in the Table of Contents.}

% \end{document}

==> notation.tex <==
\[V_{t} = \bigcup_{s=1}^{t}\big\{X_{s}\big\}\]
\[\tau_{1} = \inf\big\{t>0: X_{t} \in V_{t-1}\big\}\]
\[\sigma_{i} = \inf\big\{t>\sigma_{i-1}: X_{t} \notin V_{t-1}\big\}\]
\[\tau_{i} = \inf\big\{t>\sigma_{i}: X_{t} \in V_{t-1}\big\}\]
\[\mathbb{P}\bigg(\eta_{i} = \tau_{i} - \sigma_{i} = k \bigg| \sum_{j=1}^{i-1}\eta_{j} = m\bigg)\]
\[\mathbb{P}\bigg(\tilde{\eta_{i}} = \tilde{\tau_{i}} - \tilde{\sigma_{i}} = k \bigg| \sum_{j=1}^{i-1}\tilde{\eta_{j}} = m\bigg)\]

